Transparent Neighborhood Approximation for Text Classifier Explanation

Recent literature highlights the critical role of neighborhood construction in deriving model-agnostic explanations, with a growing trend toward deploying generative models to improve synthetic instance quality, especially for explaining text classifiers. These approaches overcome the challenges in neighborhood construction posed by the unstructured nature of texts, thereby improving the quality of explanations. However, the deployed generators are usually implemented via neural networks and lack inherent explainability, sparking arguments over the transparency of the explanation process itself. To address this limitation while preserving neighborhood quality, this paper introduces a probability-based editing method as an alternative to black-box text generators. This approach generates neighboring texts by implementing manipulations based on in-text contexts. Substituting the generator-based construction process with recursive probability-based editing, the resultant explanation method, XPROB (explainer with probability-based editing), exhibits competitive performance according to the evaluation conducted on two real-world datasets. Additionally, XPROB's fully transparent and more controllable construction process leads to superior stability compared to the generator-based explainers.

==> mainmatter/_xproa.tex <==
\section{Progressive Neighborhood Approximation with a Generative Autoencoder}
\label{sec:xproaxGen}
This section elaborates on the generator-based neighborhood construction for texts, a core component of the proposed \gbased{}.
Given a model $f(\cdot)$ and an input text $x$, the goal of an explainer is to find an explanation $\xi$, which specifies contributions of input features to the target decision\footnote{For simplicity, we assume a binary classification problem: $y\in \{+, -\}$.} $y=f(x)$.
% (a table summarizing notations used can be found in Supplement~\ref{TODO}).
In pursuit of feature attributions, \gbased{}, as a model-agnostic explainer, builds the neighborhood $N$ of an inquiry and subsequently extracts the explanation indirectly from a surrogate $g(\cdot)$ (details about the extraction are presented in Section~\ref{sec:explanationsMain}).
The surrogate model $g(\cdot)$ is trained on the pseudo-labeled neighborhood with the aim of emulating the local behavior of the black box $f(x)$.
In line with previous work~\cite{alvarez2017causal}, neighboring texts are defined as texts with similar components and meanings.

To facilitate the extraction of explanatory information, it is imperative for the surrogate to possess self-explainable property.
However, in exchange for transparency, the capacity of the surrogate is typically constrained, often taking the form of a linear model.
For the weak learner to faithfully capture the local behavior of $f(\cdot)$, it is essential that the constructed $N$ carefully locates the vicinity of $x$.
A properly constructed neighborhood highlighting only the relevant decision boundary promotes explanation quality by simplifying the imitation task for the surrogate.
% Maybe a visualization showing how this would help?

\subsection{Neighborhood Construction with Generative Autoencoder}
\label{sec:generativeModel}
% 3. Violating locality constraint --> a broader view of target model behaviors, difficult to imitate
%    --> unfaithful imitation harming explainability (again emphasize the motivation, with figure?)
% 3. To fulfill the locality constraint, two properties to possess
%    --> Reconstruction ability: first the generator should be able to reconstruct the instance of interest, 
%        otherwise, it is impossible to generate the neighborhood for $x$ if the remapping from embedding space 
%        to text space is unreliable (why some generators are inappropriate choices)
%    --> Locality preserving property: the latent space could be chaos, that encodings of irrelevant texts are
%        spatially close. In this case, neighborhoods constructed in latent space are not necessarily representing
%        neighboring texts of $x$.
In \gbased{}, the fundamental concept for enhancing neighborhood construction is the incorporation of a generative autoencoder.
A generative autoencoder $G$ consists of a deterministic encoder $E:\mathcal{X}\rightarrow\mathcal{Z}$, which maps from the text space to the latent space where neighbor sampling occurs, and a probabilistic decoder $D:\mathcal{Z}\rightarrow\mathcal{X}$, responsible for reconstructing word sequences from corresponding embeddings.
To prepare the generator for neighborhood construction, $G$ is trained on a dataset $X_G\sim\mathcal{X}$, which is sampled from the same domain as the data fed to the black box.
Please note that $X_G$ does not necessarily have intersections with the training set $X\sim\mathcal{X}$ for the classifier.
To start neighborhood construction, \gbased{}~encodes the input text $x$ with $E$.
The resultant latent representation $z=E(x)$ serves as a pivot point locating the neighborhood in the latent space.
Following encoding, a set of neighboring vectors $Z$ is sampled surrounding the pivot, and the final neighborhood $N$ is created by decoding the latent neighborhood, $N=D(Z)$.

To satisfy the locality constraint, a fundamental assumption in neighborhood construction using a generative autoencoder is that the latent neighborhood $Z$ represents the one $N$ in the text space.
For the validity of this assumption, the selected generator must fulfill two essential properties: the reconstruction property and the locality-preserving property.
The \emph{reconstruction property} requires an autoencoder to be competent in reconstructing an input text from its encoding, i.e., $x = D(E(x))$.
It ensures that the generated neighborhood is relevant to the target decision.
The \emph{locality-preserving property} refers to the generator's ability to map neighboring texts to spatially close latent vectors, and vice versa.
Combining the locality-preserving property with the previous one allows the construction to produce neighboring texts of $x$.

While there are numerous options for generators, not all of them possess the two properties.
For example, a standard VAE~\cite{bowman2016generating}, which sacrifices its reconstruction ability as a trade-off for better generative performance~\cite{song2019latent, dai2020usual}, yields less contextually related texts as shown in Section~\ref{sec:dependency}.
In this work, we employ DAAE~\cite{shen2020educating}, a generator that learns locality-preserving latent space by augmenting an adversarial autoencoder with a denoising objective.
The denoising objective requires the generator to reconstruct original texts from their perturbed versions, encouraging the model to map similar texts to similar latent representations since they share perturbed variants.
This, in turn, contributes to both the reconstruction and locality-preserving properties.
The well-structured latent space geometry facilitates the generation of high-quality neighboring texts and finally promotes the quality of explanations.

\subsection{Progressive Neighborhood Approximation}
\label{sec:neighborhoodGeneration}
With the generator determined, we detail the progressive neighborhood approximation for latent space sampling.
When given an inquiry $x$ and its latent vector $z$, \gbased{}~initializes the neighborhood with a corpus $X_L$, which is down-sampled from the generator training set.
The corpus helps the construction process adapt to the underlying data distribution.
More specifically, \gbased{}~draws the $k$-closest counterfactuals, which are instances with a different pseudo label than $f(x)$, from $X_L$ according to their latent space distances to $z$.
The latent representations of the chosen counterfactuals collectively form a landmark set $L$.
These instances are referred to as \textit{landmarks} because they are the closest known counterfactuals that highlight the local decision boundary.

After neighborhood initialization, the proposed progressive neighborhood approximation (Algorithm~\ref{alg:construct}) proceeds to construct the neighborhood for the inquiry through an iterative process.
This iterative process seeks to discover and exploit closer counterfactuals of $x$, continuing until the termination criterion is met, e.g. when no closer counterfactual is found in successive iterations or the repeating count reaches its limitation.
During each iteration, the approximation repeatedly collects the closest counterfactual $z_c$ (lines 4-8), which is generated by the two-stage interpolation (line 5), as landmarks for the next generation (line 6).
The process is repeated until a sufficient number of landmarks is obtained (line 8).
All intermediate texts produced during the repeated process are added to $N$ (line 7) as candidates for the final neighborhood.
Once the termination criterion is met, the approach finalizes the neighborhood by selecting the $n$ closest texts from the candidate pool (line 11).

\begin{algorithm}[tb]
\caption{Progressive Neighborhood Approximation}
\label{alg:construct}
\begin{algorithmic}[1]
\REQUIRE $x$: inquired text; $z$: encoding of $x$; $L$: landmarks % landmark
\ENSURE  $N$: neighborhood of $x$

\STATE $N=\varnothing$
\WHILE{terminate criterion NOT met}
    \STATE $L_{\mathit{new}}=\varnothing$
    \REPEAT
        \STATE $N_{new}, z_c = \mathrm{TwoStageInterpolation}(x, z, L)$
        \STATE $L_{\mathit{new}}.\mathrm{add}(z_c)$
        \STATE $N=N\cup N_{\mathit{new}}$
    \UNTIL{$|L_{\mathit{new}}|=k$}    
    \STATE $L=L_{\mathit{new}}$
\ENDWHILE
\STATE $N=\mathrm{Closest}(N, n)$ \COMMENT{\textit{finalize $N$ with the closest texts}}
\RETURN $N$ 
\end{algorithmic} 
\end{algorithm}

At the core of the approximation process, the two-stage interpolation presented in Algorithm~\ref{alg:approximate} takes the inquired text and the up-to-date landmark set as inputs and returns the interpolated texts along with the latent representation of the closest counterfactual.
As the name implies, the approach comprises two stages of interpolation, a common operation in autoencoder-based text generation~\cite{bowman2016generating}, defined as follows:
\begin{equation}
I(z_a, z_b)=\{z_i \mid z_i=z_a+i\cdot \frac{(z_a-z_b)}{s+1}, 1\leq i\leq s\} \label{interpolate}
\end{equation}
The operation interpolates $s$ instances uniformly between two given latent vectors, implementing successive and meaningful text manipulations.
The first stage (line 3) conducts interpolation between two samples drawn from $L$ (line 2), thereby increasing the variety of counterfactuals for neighborhood exploration.
After filtering out instances with the same label as $x$ (line 4), the second stage interpolates between the pivot and each of the newly generated counterfactuals (lines 5, 6).
The interpolation between poles having different pseudo labels highlights the local decision boundary that lies in between.

Compared to random latent space sampling, the progressive neighborhood approximation efficiently explores the latent space with the two-stage interpolation along manipulation directions that have the most significant impact on model outcomes.
Furthermore, its neighborhood initialization with counterfactuals overcomes the dependency on manually defined search ranges, the optimal value of which can vary when explaining different decisions.
As a result, through the iterative process, \gbased{}~constructs a neighborhood with realistic neighboring texts.
These factual and counterfactual instances highlight the local decision boundary relevant to the inquired decision. 

\begin{algorithm}[tb]
\caption{Two-stage Interpolation}
\label{alg:approximate}
\begin{algorithmic}[1]
\REQUIRE $x$: inquired text; $z$: encoding of $x$; $L$: landmarks % landmark
\ENSURE  $N_{\mathit{new}}$: new neighbors; $z_c$: the closest counterfactual

\STATE $Z=\varnothing$
\STATE $z_p, z_q = \mathrm{RandomlyDraw}(L, 2)$ % \\ \COMMENT{\textit{draw randomly 2 vectors from the landmark set}}
\STATE $Z'=I(z_p,z_q)$ \COMMENT{\textit{1st interpolation: between landmarks}}
\STATE $Z_{c} = \{z_i | z_i\in Z', f(D(z_i))\neq f(x)\}$    \COMMENT{\textit{counterfactuals}}

\FOR{$z_i\in Z_{c}$}
    \STATE $Z = Z \cup I(z_i, z)$ \COMMENT{\textit{2nd interpolation: between poles}}
\ENDFOR

\STATE $N_{\mathit{new}} = D(Z)$
% \STATE $z_c=\underset{z_i\in Z_c}{\argmin}~d(z_i, z)$ \COMMENT{distance between latent vectors}
\STATE $z_c=\argmin_{z_i \in Z_c}d(z_i, z)$ \COMMENT{\textit{distance to the pivot}}
\RETURN $N_{\mathit{new}}, z_c$    % Each two-stage interpolation produces a seed as a landmark for next generation
\end{algorithmic} 
\end{algorithm}

==> mainmatter/bak_examples.tex <==
    % \multicolumn{3}{p{.975\textwidth}}{\textbf{Input}: maybe got a bad one? \hfill Dataset: \textbf{Amazon}, \textbf{RF} $b(\cdot)$: {\textcolor{red}{0.9}}\Tstrut}
    % \\[0.2em] \hline
    % \\[-1em] \multirow{2}{*}[-3em]{\textbf{\gbased{}}} &
    % \textbf{Saliency}: maybe got a \hlRed[0.3]{bad} one? &
    % \textbf{Extrinsic words}: \hlBlue[0.27]{good} \hlBlue[0.15]{great}\\
    % & \textbf{Factuals}: & \textbf{Counterfactuals}: \\
    % & 1) maybe what got a bad one ? & 1) maybe what got a good one ?\\
    % & 2) maybe it was a bad one & 2) would have bought this one ...\\
    % & 3) maybe got a bad one ! & 3) once you got a one ...\\
    % & 4) was there a bad thing ? & 4) good luck getting a <unk> one !\\
    % & 5) maybe i got something a bad one & 5) maybe i m a good one
    % \\[0.2em] \hline
    % \\[-1em] \multirow{2}{*}[-3em]{\textbf{\pbased{}}} &
    % \textbf{Saliency}: maybe got a \hlRed[0.31]{bad} one? &
    % \textbf{Extrinsic words}: \hlBlue[0.19]{best} \hlBlue[0.16]{perfect} \hlBlue[0.16]{good}\\
    % & \textbf{Factuals}: & \textbf{Counterfactuals}: \\
    % & 1) maybe got good bad for one & 1) maybe got a good film for one\\
    % & 2) bad maybe got time & 2) got a bad maybe the best series of all time\\
    % & 3) maybe got my item ! one a bad & 3) maybe you have got to read this one !\\
    % & 4) one maybe got just as a bad review & 4) got one good great maybe the best yeah ! bad ?\\
    % & 5) got for one ? maybe & 5) got one well ... maybe for kids ... ?
    % \\[0.2em] \hline \multicolumn{3}{c}{} \\[-0.3em] \hline

    % \rowcolor{Gray}
    % \multicolumn{3}{p{17.7cm}}{\textbf{Input}: broke within $\langle num\rangle$ uses \hfill Dataset: \textbf{Amazon}, \textbf{RF} $b(\cdot)$: {\textcolor{red}{0.9}}\Tstrut}
    % \\[0.2em] \hline
    % \\[-1em] \multirow{2}{*}[-3em]{\textbf{\gbased{}}} &
    % \textbf{Saliency}: \hlRed[0.39]{broke} within $\langle num\rangle$ uses &
    % \textbf{Extrinsic words}: \hlBlue[0.27]{great} \hlRed[0.16]{no}\\
    % & \textbf{Factuals}: & \textbf{Counterfactuals}: \\
    % & 1) broke within few uses & 1) great within the past\\
    % & 2) broke from the past & 2) very slow within $\langle num\rangle$\\
    % & 3) broke within $\langle num\rangle$ uses $\langle num\rangle$ of $\langle unk\rangle$ drive & 3) blade within the final\\
    % & 4) broke within $\langle num\rangle$ uses of & 4) woh the $\langle num\rangle$ hours of watching\\
    % & 5) broke within the dozen & 5) died within a week
    % \\[0.2em] \hline
    % \\[-1em] \multirow{2}{*}[-3em]{\textbf{\pbased{}}} &
    % \textbf{Saliency}: \hlRed[0.29]{broke} within $\langle num\rangle$ uses &
    % \textbf{Extrinsic words}: \hlBlue[0.23]{great} \hlBlue[0.14]{good} \hlBlue[0.13]{excellent}\\
    % & \textbf{Factuals}: & \textbf{Counterfactuals}: \\
    % & 1) broke within $\langle num\rangle$ uses & 1) within $\langle num\rangle$ uses\\
    % & 2) uses broke within $\langle num\rangle$ & 2) good sound, but broke within\\
    % & 3) broke within book $\langle num\rangle$ uses & 3) great item with lots of uses broke within $\langle num\rangle$\\
    % & 4) uses, but broke within $\langle num\rangle$ & 4) my daughter loves it and uses it broke within a $\langle num\rangle$\\
    % & 5) uses broke within & 5) $\langle num\rangle$ uses great until the clip broke within
    % \\[0.2em] \hline \multicolumn{3}{c}{} \\[-0.3em] \hline

    

==> mainmatter/sup_longtable.tex <==
\begin{center}
    % \centering
    \begin{footnotesize}
        \begin{longtable}{p{0.47\textwidth} p{0.48\textwidth}} 
            \caption{Example explanations on different classifiers by \gbased{}, \pbased{}}\\
            \hline
            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: why you shouldn't take reviews seriously \hfill Dataset: \textbf{Amazon}, \textbf{RF} $b(\cdot)$: {\textcolor{red}{0.72}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em] 
            \textbf{Saliency}: \hlRed[0.16]{why} you shouldn't take reviews seriously &
            \textbf{Extrinsic words}: \hlBlue[0.19]{must} \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) why you shouldn't take reviews seriously seriously & 1) why you shouldn't read this seriously\\
            2) why can't take you reviews seriously? & 2) why must you won't write reviews\\
            3) why can't take this reviews seriously & 3) who think that s take on reviews seriously make\\
            4) why s you shouldn't use reviews seriously & 4) why can't take the good script to seriously\\
            5) why you shouldn't write reviews seriously & 5) why can't you write good reviews
            \\[0.38em] \hline \\[-1em] 
            \textbf{Saliency}: \hlRed[0.15]{why} you shouldn't take reviews seriously &
            \textbf{Extrinsic words}: \hlBlue[0.21]{best} \hlBlue[0.19]{great} \hlBlue[0.13]{love} \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) shouldn why take the reviews. seriously & 1) shouldn't take reviews! seriously\\
            2) why you shouldn't take a pa of reviews with you seriously & 2) shouldn't why you will take a pa of reviews with you seriously\\
            3) you shouldn't take reviews! why & 3) great reviews but why i shouldn't you really take it that seriously\\
            4) you why read the reviews seriously. shouldn't & 4) take you why this simple shouldn't sound this good reviews seriously\\
            5) why t take reviews! seriously & 5) shouldn't take seriously. one of why the best albums i own reviews!
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline

            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: the longest $\langle num\rangle$ minutes in my life \hfill Dataset: \textbf{Amazon}, \textbf{RF} $b(\cdot)$: {\textcolor{blue}{0.65}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: the \hlBlue[0.12]{longest} $\langle num\rangle$ minutes in my \hlBlue[0.09]{life} &
            \textbf{Extrinsic words}: \hlRed[0.35]{worst} \hlRed[0.21]{waste} \hlRed[0.18]{after} \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the longest $\langle num\rangle$ minutes of my life back & 1) the longest $\langle num\rangle$ minutes after life in my mouth\\
            2) the longest six minutes in my life! & 2) a waste of $\langle num\rangle$ hours of my life\\
            3) the longest movie i have in my life & 3) the longest generation $\langle num\rangle$ you in in my disappointment\\
            4) the longest $\langle num\rangle$ minutes of my life & 4) the worst comedy of all time in my life\\
            5) the longest $\langle num\rangle$ minutes i in my life & 5) not the $\langle num\rangle$ minutes of your life
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: the longest $\langle num\rangle$ minutes in my \hlBlue[0.12]{life} &
            \textbf{Extrinsic words}: \hlRed[0.2]{worst} \hlRed[0.17]{waste} \hlRed[0.13]{after} \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the longest $\langle num\rangle$ minutes of my life & 1) this is the longest $\langle num\rangle$ minutes\\
            2) in the longest $\langle num\rangle$ minutes $\langle num\rangle$ life & 2) in a waste of $\langle num\rangle$ minutes of my life\\
            3) in the longest! my $\langle num\rangle$ & 3) in the longest! $\langle num\rangle$\\
            4) my life in $\langle num\rangle$ minutes & 4) in the longest $\langle num\rangle$ minutes of my life i ll never get back\\
            5) the longest! my $\langle num\rangle$ minutes & 5) my life $\langle num\rangle$ stars for the longest $\langle num\rangle$ minutes! 
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline
        
            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: the best movie ever! harry, hermione and ron are amazing \hfill Dataset: \textbf{Amazon}, \textbf{RF} $b(\cdot)$: {\textcolor{blue}{0.86}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em] 
            \textbf{Saliency}: the \hlBlue[0.4]{best} movie ever! harry, hermione and ron are \hlBlue[0.06]{amazing} &
            \textbf{Extrinsic words}: \hlRed[0.31]{worst} \hlRed[0.21]{not} \hlRed[0.12]{boring} \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the best movie ever! harry potter $\langle unk\rangle$ and ron, amazing! & 1) the worst movie ever, harry potter and $\langle unk\rangle$ are quite wrong\\
            2) the best movie ever! harry potter and $\langle unk\rangle$ sean is original & 2) the worst movie ever ! harry potter $\langle unk\rangle$ and james $\langle unk\rangle$ is\\
            3) the best movie ever! harry potter and $\langle unk\rangle$ sean are amazing & 3) the worst harry potter movie and harry potter was awful\\
            4) the best movie ever! harry potter $\langle unk\rangle$ and ron is quite amazing & 4) the worst movie ever liked this, and $\langle unk\rangle$ were done.\\
            5) the best movie ever! harry potter and $\langle unk\rangle$ sean james! & 5) the worst robin cook ever $\langle unk\rangle$ and ron ever
            \\[0.2em] \hline
            \\[-1em] 
            \textbf{Saliency}: the \hlBlue[0.31]{best} movie ever! harry, hermione and ron are \hlBlue[0.07]{amazing} &
            \textbf{Extrinsic words}: \hlRed[0.43]{worst} \hlRed[0.12]{bad} \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the best harry, hermione the best movie ever. ron & 1) ron are the worst movie ever made... harry really, hermione ever\\
            2) are amazing movie, hermione ever! harry!!!!!!!!! & 2) ron are amazing the best worst movie i have ever! harry\\
            3) ron are. and the movie, ever. & 3) amazing the worst. movie, hermione ever.\\
            4) amazing the best horror movie, hermione the best harry. ron & 4) the best worst. ron movie, hermione ever.\\
            5) are and ron movie, hermione ever & 5) harry is amazing, ron movie ever is beyond bad!
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline
        
            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: don't waste your time or money on this one \hfill Dataset: \textbf{Amazon}, \textbf{LSTM} $b(\cdot)$: {\textcolor{red}{0.93}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: don't \hlRed[0.25]{waste} your time or \hlRed[0.2]{money} on this one &
            \textbf{Extrinsic words}: \hlRed[0.22]{skip} \hlRed[0.19]{not} \hlBlue[0.14]{best} \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) don't waste your time or money on this one on this & 1) don't read any time or $\langle unk\rangle$ on this one!\\
            2) don't waste your time or money for this out & 2) don't last time or time on this album\\
            3) make a waste of your time training on the planet & 3) great book for any time or for money on this\\
            4) don't waste your time or money, don t buy this & 4) don't know your time for your projector and this one\\
            5) i don't waste your time or money on this one & 5) the eagles must have your old people on this one
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: don t \hlRed[0.3]{waste} your time or \hlRed[0.18]{money} on this one &
            \textbf{Extrinsic words}: \hlBlue[0.12]{great} \hlBlue[0.1]{best} \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) waste your money on this one time or don & 1) this one of waste your time money on, or don't, a sequal to a great movie\\
            2) waste your money on this one time or don't & 2) this one of his best one on your time money or two! don\\
            3) waste your time money on this one or don & 3) on this the perfect t waste one of your time or!\\
            4) money this one or on don't waste your time & 4) this on a great value for your time or money don\\
            5) your money on this one time or don't waste & 5) don't waste your time with this one, read a good book.
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline
        
            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: it shouldn't be sold. \hfill Dataset: \textbf{Amazon}, \textbf{LSTM} $b(\cdot)$: {\textcolor{red}{0.95}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it \hlRed[0.23]{shouldn't} be \hlRed[0.16]{sold}. &
            \textbf{Extrinsic words}: \hlRed[0.26]{disappointing} \hlRed[0.22]{not} \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) it shouldn't be sold out. & 1) a masterpiece that should be not.\\
            2) there shouldn't be sold & 2) it s passable but better now!\\
            3) it shouldn't be used. & 3) there must be $\langle num\rangle$.\\
            4) it shouldn't be meant to. & 4) it might be available for its $\langle unk\rangle$.\\
            5) it shouldn't be sold for. & 5) this book should be available made!
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it \hlRed[0.1]{shouldn't} be \hlRed[0.16]{sold}. &
            \textbf{Extrinsic words}: \hlBlue[0.2]{good} \hlBlue[0.09]{must} \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) shouldn't it be sold. & 1) shouldn it. must be good...\\
            2) shouldn't sold. it be & 2) sold it d be a great collection if...\\
            3) it shouldn't be sold. & 3) it this terrific book shouldn't be sold a civil war novel\\
            4) it shouldn't be. sold & 4) it has gbv sold out? i shouldn't be... this is a great album.\\
            5) shouldn sold it. be... & 5) shouldn't it is to be, it. s up to me!
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline
        
            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: good small poion homemade icecream \hfill Dataset: \textbf{Amazon}, \textbf{LSTM} $b(\cdot)$: {\textcolor{blue}{0.92}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: \hlBlue[0.26]{good} \hlRed[0.15]{small} poion homemade icecream &
            \textbf{Extrinsic words}: \hlRed[0.28]{ruined} \hlRed[0.23]{inadequate} \hlRed[0.22]{not} \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) good small sized $\langle unk\rangle$ soup & 1) good small piece of dutch\\
            2) good small formula type $\langle unk\rangle$ & 2) good small sized type $\langle unk\rangle$\\
            3) good small sized $\langle unk\rangle$ homemade & 3) good value and ruined by foul $\langle unk\rangle$\\
            4) good small pen type $\langle unk\rangle$ & 4) very small sized ruined $\langle unk\rangle$\\
            5) good bit overwhelming $\langle unk\rangle$ & 5) $\langle unk\rangle$ small sized $\langle unk\rangle$
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: \hlBlue[0.31]{good} \hlRed[0.13]{small} poion \hlBlue[0.1]{homemade} icecream &
            \textbf{Extrinsic words}: \hlRed[0.26]{too} \hlRed[0.25]{runs} \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) good small poion homemade icecream & 1) small poion homemade\\
            2) good small poion homemade & 2) good too small poion homemade\\
            3) good to small poion homemade icecream & 3) good content but small poion i didn't know it was homemade icecream\\
            4) good for small poion homemade & 4) only the small poion homemade\\
            5) good it s a small poion homemade & 5) good way too small poion homemade
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline

            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: it's full of fresh ingredients, light and tasty. \hfill Dataset: \textbf{Yelp}, \textbf{RF} $b(\cdot)$: {\textcolor{blue}{0.88}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it's full of \hlBlue[0.25]{fresh} ingredients, light and \hlBlue[0.15]{tasty}. &
            \textbf{Extrinsic words}: \hlRed[0.48]{not} \hlBlue[0.14]{delicious} \hlBlue[0.14]{wood}
             \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) it's full of ingredients, light and tasty food. & 1) it's full of ingredients, ingredients and light salad.\\
            2) it's full of ingredients, fresh light and tasty. & 2) it's full of ingredients, just light food.\\
            3) it was full of fresh ingredients, light and tasty. & 3) i ate different variety of ingredients and light salad.\\
            4) it's full of fresh ingredients, light and tasty variety. & 4) it's full of all ingredients and light groups.\\
            5) it's full of ingredients and light on food. & 5) it's full of ingredients, not light and tasty.
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it's full of \hlBlue[0.26]{fresh} ingredients, light \hlBlue[0.18]{and} \hlBlue[0.13]{tasty}. &
            \textbf{Extrinsic words}: \hlRed[0.41]{\textlangle \textit{num}\textrangle} \hlRed[0.12]{was} \hlRed[0.1]{over}
             \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) full of it was light and fresh ingredients. & 1) light of the ingredients are full!!!.\\
            2) light of our breakfast was tasty tasty tasty and fresh ingredients. & 2) of it tasty fresh, wasn't tasty/fresh enough to have been over \$$\langle num\rangle$.\\
            3) full of fresh tasty. & 3) it was light and ingredients.\\
            4) it and they have a full of ingredients, light,. & 4) light was full, tasty's.\\
            5) light was tasty fresh ingredients. & 5) it $\langle num\rangle$ fresh, and fresh, fresh ingredients.
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline
            
            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: it was super dry and had a weird taste to the entire slice. \hfill Dataset: \textbf{Yelp}, \textbf{RF} $b(\cdot)$: {\textcolor{red}{0.81}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it was super \hlRed[0.15]{dry} and had a weird taste to the entire slice. &
            \textbf{Extrinsic words}: \hlBlue[0.35]{delicious} \hlBlue[0.32]{nice} \hlBlue[0.29]{good}
             \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) it was super dry and had a weird taste and the whole slice. & 1) it was super dry and had a good taste to the entire slice.\\
            2) it was super dry and had a weird taste of the whole plate. & 2) it was super good and had a weird taste to my half slice.\\
            3) it was super dry and had a weird taste to my half slice. & 3) it was very dry and had a good taste of the whole plate.\\
            4) it was super dry and had a taste flavor to the whole slice. & 4) and it was totally the flavor of the meal.\\
            5) it was super dry and had a weird taste to my whole slice. & 5) it was super dry and had a nice taste of the entire slice.
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it \hlRed[0.15]{was} super \hlRed[0.19]{dry} \hlBlue[0.21]{and} had a \hlRed[0.13]{weird} taste to the entire slice. &
            \textbf{Extrinsic words}: \hlBlue[0.46]{great} \hlBlue[0.28]{delicious} \hlBlue[0.27]{good}
             \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) slice was the entire people here are super weird and taste. & 1) entire a super weird, taste.\\
            2) i had to the dry and it was a weird. & 2) dry and slice.\\
            3) to it dry food taste a slice & 3) entire slice and had to it was super good.\\
            4) entire it had was a weird, but was n't super dry. & 4) it and had the taste was very weird.\\
            5) and it to the entire taste was dry! & 5) super dry and slice.
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline

            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: the food is excellent and the service is exceptional! \hfill Dataset: \textbf{Yelp}, \textbf{RF} $b(\cdot)$: {\textcolor{blue}{0.96}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: the food is \hlBlue[0.24]{excellent} \hlBlue[0.19]{and} the \hlBlue[0.08]{service} is \hlBlue[0.11]{exceptional}! &
            \textbf{Extrinsic words}: \hlRed[0.35]{not} \hlRed[0.17]{horrible} \hlRed[0.16]{awful}
             \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the food is excellent and the service is superb! & 1) the food is good, and not service at all.\\
            2) the food is excellent, and the service is phenomenal! & 2) the food is not incredible and the service is mediocre at best.\\
            3) the food is excellent and the service is exceptional at best & 3) the food is satisfying and the bill was exceptional.\\
            4) the food is excellent and the service is at! & 4) the food, oh my, the room was/is fabulous.\\
            5) the food is excellent and the service was exceptional. & 5) the food is horrible and the service is bad!!
            \\[0.2em] \hline            
            \\[-1em]
            \textbf{Saliency}: the food is \hlBlue[0.3]{excellent} \hlBlue[0.17]{and} the service is exceptional! &
            \textbf{Extrinsic words}: \hlRed[0.11]{nothing} \hlRed[0.09]{average}
             \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) excellent food and the service is exceptional. & 1) is the food service was exceptional!.\\
            2) is the food?! & 2) the $\langle num\rangle$ star is for the appetizer and the server's excellent service.\\
            3) excellent and the exceptional service is. & 3) the service is exceptional.\\
            4) excellent food is average and the service is exceptional. & 4) the food is ok... but the service is exceptional.\\
            5) excellent and is the food exceptional & 5) the food is nothing exceptional!
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline

            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: the cake portion was extremely light and a bit dry. \hfill Dataset: \textbf{Yelp}, \textbf{LSTM} $b(\cdot)$: {\textcolor{blue}{0.7}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: the cake portion was extremely \hlBlue[0.33]{light} and a bit \hlRed[0.27]{dry}. &
            \textbf{Extrinsic words}: \hlBlue[0.36]{tasty} \hlBlue[0.3]{awesome} \hlBlue[0.29]{generous}
             \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the cake was extremely generous and a light over dry tuna. & 1) the cake was extremely large and a bit over dry.\\
            2) the cake portion is large and heavy to a smooth. & 2) the cake portion was extremely light and a tad dry.\\
            3) the cake itself was extremely light and a bit dry. & 3) the cake portion was extremely large and a bit dry.\\
            4) the cake cake was extremely tasty and a gummy dry. & 4) the cake portion was extremely light and a dry dry.\\
            5) the cake portion was extremely thick and a light dry. & 5) the cake was extremely small and light in a dry.
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: the \hlBlue[0.09]{cake} portion was extremely \hlBlue[0.33]{light} and a bit \hlRed[0.46]{dry}. &
            \textbf{Extrinsic words}: \hlBlue[0.22]{best} \hlRed[0.22]{however}
             \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) the cake was extremely light and a bit dry. & 1) and the cake portion was extremely dry.\\
            2) extremely portion - & 2) light was a bit dry.\\
            3) the portion was bit dry and light, at best cake. & 3) the cake portion was a bit.\\
            4) the cake portion was light. & 4) portion is extremely dry and a light.\\
            5) crust is extremely dry and portion was a light. & 5) light and the cake was bit dry.
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline

            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: it was super dry and had a weird taste to the entire slice. \hfill Dataset: \textbf{Yelp}, \textbf{LSTM} $b(\cdot)$: {\textcolor{red}{1.0}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it was \hlBlue[0.08]{super} \hlRed[0.45]{dry} and had a \hlRed[0.17]{weird} \hlRed[0.17]{taste} to the entire slice. &
            \textbf{Extrinsic words}: \hlBlue[0.4]{great} \hlBlue[0.3]{delicious} \hlRed[0.24]{sour}
             \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) it was super dry and had a weird taste to the whole slice. & 1) it was super dry and had a sweet flavor to the entire combination.\\
            2) it was super dry and had a weird taste to my half slice. & 2) it was perfectly cooked and had a flavor taste and the whole.\\
            3) it was super dry and had a nice taste of the entire slice. & 3) very dry and had a good flavor to a nice slice of the strip\\
            4) it was perfectly dry and had a flavor taste and the whole. & 4) it was super awesome and had the $\langle unk\rangle$ taste to the half.\\
            5) it was super dry and had a weird taste to the half. & 5) it was so good and had a flavor to the whole dish.
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: it was \hlBlue[0.25]{super} \hlRed[0.27]{dry} \hlBlue[0.09]{and} had a \hlRed[0.23]{weird} taste to the entire slice. &
            \textbf{Extrinsic words}: \hlBlue[0.34]{great} \hlBlue[0.33]{fresh} \hlBlue[0.29]{good}
             \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) super dry it is weird to slice at and delicious to taste. & 1) slice it was the entire super good dry.\\
            2) had the entire way you slice it was weird. & 2) weird and a great taste.\\
            3) to and the taste was a super dry. & 3) entire slice i super loved it had dry.\\
            4) entire a super weird. & 4) slice and it was super fresh taste weird.\\
            5) had to the taste was a slice. & 5) entire and it was super fresh taste weird.
            \\[0.2em] \hline \multicolumn{2}{c}{} \\[-0.5em] \hline

            \rowcolor{Gray}
            \multicolumn{2}{p{.975\textwidth}}{\textbf{Input}: but service was horrible both times. \hfill Dataset: \textbf{Yelp}, \textbf{LSTM} $b(\cdot)$: {\textcolor{red}{1.0}}\Tstrut}
            \\[0.2em] \hline
            \\[-1em]
            \textbf{Saliency}: \hlRed[0.1]{but} service was \hlRed[0.69]{horrible} \hlBlue[0.11]{both} times. &
            \textbf{Extrinsic words}: \hlRed[0.44]{disappointing} \hlRed[0.42]{different} \hlBlue[0.3]{excellent}
             \hfill \textbf{\gbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) but the service was horrible times. & 1) but the service was enjoyed each.\\
            2) but service was horrible both times times. & 2) but it was friendly and both times.\\
            3) but service was horrible and both times. & 3) but the service was always friendly times.\\
            4) but service was horrible and times. & 4) but service was truly enjoyed times.\\
            5) but it was horrible both times. & 5) the service was friendly and prompt.
            \\[0.2em] \hline
            
            \\[-1em]
            \textbf{Saliency}: but service was \hlRed[0.65]{horrible} \hlBlue[0.16]{both} times. &
            \textbf{Extrinsic words}: \hlBlue[0.3]{super} \hlBlue[0.23]{great}
             \hfill \textbf{\pbased{}}\\
            \textbf{Factuals}: & \textbf{Counterfactuals}: \\
            1) both times but was horrible service & 1) but horrible service was both times are great!\\
            2) but service was horrible both times! & 2) both times was but service\\
            3) both times was horrible but service & 3) service was horrible but both delicious!\\
            4) service was horrible but both times! & 4) horrible both good food + good service = good times.\\
            5) service but was horrible both times! & 5) both times, great food but super horrible service was!
            \\[0.2em] \hline 
            \label{tab:appendix_quality}
        \end{longtable}
    \end{footnotesize}
\end{center}
